ARMP: Autoregressive Motion Planning for Quadruped Locomotion and Navigation in Complex Indoor Environments

Generating natural and physically feasible motions for legged robots has been a challenging problem due to its complex dynamics. In this work, we introduce a novel learning-based framework of autoregressive motion planner (ARMP) for quadruped locomotion and navigation. Our method can generate motion plans with an arbitrary length in an autoregressive fashion, unlike most offline trajectory optimization algorithms for a fixed trajectory length. To this end, we first construct the motion library by solving a dense set of trajectory optimization problems for diverse scenarios and parameter settings. Then we learn the motion manifold from the dataset in a supervised learning fashion. We show that the proposed ARMP can generate physically plausible motions for various tasks and situations. We also showcase that our method can be successfully integrated with the recent robot navigation frameworks as a low-level controller and unleash the full capability of legged robots for complex indoor navigation.

==> 00.bibliography.bib.tex <==
\begin{thebibliography}{99}
@article{kareer2022vinl,
  title={ViNL: Visual Navigation and Locomotion Over Obstacles},
  author={Kareer, Simar and Yokoyama, Naoki and Batra, Dhruv and Ha, Sehoon and Truong, Joanne},
  journal={arXiv preprint arXiv:2210.14791},
  year={2022}
}

@inproceedings{truong2021learning,
  title={Learning navigation skills for legged robots with learned robot embeddings},
  author={Truong, Joanne and Yarats, Denis and Li, Tianyu and Meier, Franziska and Chernova, Sonia and Batra, Dhruv and Rai, Akshara},
  booktitle={2021 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
  pages={484--491},
  year={2021},
  organization={IEEE}
}

@article{truong2022rethinking,
  title={Rethinking sim2real: Lower fidelity simulation leads to higher sim2real transfer in navigation},
  author={Truong, Joanne and Rudolph, Max and Yokoyama, Naoki and Chernova, Sonia and Batra, Dhruv and Rai, Akshara},
  journal={arXiv preprint arXiv:2207.10821},
  year={2022}
}

@article{peng2018deepmimic,
  title={Deepmimic: Example-guided deep reinforcement learning of physics-based character skills},
  author={Peng, Xue Bin and Abbeel, Pieter and Levine, Sergey and Van de Panne, Michiel},
  journal={ACM Transactions On Graphics (TOG)},
  volume={37},
  number={4},
  pages={1--14},
  year={2018},
  publisher={ACM New York, NY, USA}
}

@article{fuchioka2022opt,
  title={OPT-Mimic: Imitation of Optimized Trajectories for Dynamic Quadruped Behaviors},
  author={Fuchioka, Yuni and Xie, Zhaoming and van de Panne, Michiel},
  journal={arXiv preprint arXiv:2210.01247},
  year={2022}
}

% References for Motion Planning
% TOWR
@article{winkler2018gait,
  title={Gait and trajectory optimization for legged systems through phase-based end-effector parameterization},
  author={Winkler, Alexander W and Bellicoso, C Dario and Hutter, Marco and Buchli, Jonas},
  journal={IEEE Robotics and Automation Letters},
  volume={3},
  number={3},
  pages={1560--1567},
  year={2018},
  publisher={IEEE}
}

% inverted pendulum model
@article{green2021learning,
  title={Learning spring mass locomotion: Guiding policies with a reduced-order model},
  author={Green, Kevin and Godse, Yesh and Dao, Jeremy and Hatton, Ross L and Fern, Alan and Hurst, Jonathan},
  journal={IEEE Robotics and Automation Letters},
  volume={6},
  number={2},
  pages={3926--3932},
  year={2021},
  publisher={IEEE}
}

% SRBD model
@inproceedings{ding2019real,
  title={Real-time model predictive control for versatile dynamic motions in quadrupedal robots},
  author={Ding, Yanran and Pandala, Abhishek and Park, Hae-Won},
  booktitle={2019 International Conference on Robotics and Automation (ICRA)},
  pages={8484--8490},
  year={2019},
  organization={IEEE}
}

% Cheetah, using SRBD.
@inproceedings{di2018dynamic,
  title={Dynamic locomotion in the mit cheetah 3 through convex model-predictive control},
  author={Di Carlo, Jared and Wensing, Patrick M and Katz, Benjamin and Bledt, Gerardo and Kim, Sangbae},
  booktitle={2018 IEEE/RSJ international conference on intelligent robots and systems (IROS)},
  pages={1--9},
  year={2018},
  organization={IEEE}
}

% Glide
@inproceedings{xie2022glide,
  title={Glide: Generalizable quadrupedal locomotion in diverse environments with a centroidal model},
  author={Xie, Zhaoming and Da, Xingye and Babich, Buck and Garg, Animesh and de Panne, Michiel van},
  booktitle={Algorithmic Foundations of Robotics XV: Proceedings of the Fifteenth Workshop on the Algorithmic Foundations of Robotics},
  pages={523--539},
  year={2022},
  organization={Springer}
}

% Falling Cat
@inproceedings{kurtz2022mini,
  title={Mini cheetah, the falling cat: A case study in machine learning and trajectory optimization for robot acrobatics},
  author={Kurtz, Vince and Li, He and Wensing, Patrick M and Lin, Hai},
  booktitle={2022 International Conference on Robotics and Automation (ICRA)},
  pages={4635--4641},
  year={2022},
  organization={IEEE}
}

% Warm start
@inproceedings{mansard2018using,
  title={Using a memory of motion to efficiently warm-start a nonlinear predictive controller},
  author={Mansard, Nicolas and DelPrete, Andrea and Geisert, Mathieu and Tonneau, Steve and Stasse, Olivier},
  booktitle={2018 IEEE International Conference on Robotics and Automation (ICRA)},
  pages={2986--2993},
  year={2018},
  organization={IEEE}
}

% Character Animation
% PFNN
@article{holden2017phase,
  title={Phase-functioned neural networks for character control},
  author={Holden, Daniel and Komura, Taku and Saito, Jun},
  journal={ACM Transactions on Graphics (TOG)},
  volume={36},
  number={4},
  pages={1--13},
  year={2017},
  publisher={ACM New York, NY, USA}
}

% MANN
@article{zhang2018mode,
  title={Mode-adaptive neural networks for quadruped motion control},
  author={Zhang, He and Starke, Sebastian and Komura, Taku and Saito, Jun},
  journal={ACM Transactions on Graphics (TOG)},
  volume={37},
  number={4},
  pages={1--11},
  year={2018},
  publisher={ACM New York, NY, USA}
}

% NSM
@article{starke2019neural,
  title={Neural state machine for character-scene interactions.},
  author={Starke, Sebastian and Zhang, He and Komura, Taku and Saito, Jun},
  journal={ACM Trans. Graph.},
  volume={38},
  number={6},
  pages={209--1},
  year={2019}
}

% LocalMotionPhase
@article{starke2020local,
  title={Local motion phases for learning multi-contact character movements},
  author={Starke, Sebastian and Zhao, Yiwei and Komura, Taku and Zaman, Kazi},
  journal={ACM Transactions on Graphics (TOG)},
  volume={39},
  number={4},
  pages={54--1},
  year={2020},
  publisher={ACM New York, NY, USA}
}


% NN manifold
@incollection{holden2015learning,
  title={Learning motion manifolds with convolutional autoencoders},
  author={Holden, Daniel and Saito, Jun and Komura, Taku and Joyce, Thomas},
  booktitle={SIGGRAPH Asia 2015 technical briefs},
  pages={1--4},
  year={2015}
}

% NN manifold + control
@article{holden2016deep,
  title={A deep learning framework for character motion synthesis and editing},
  author={Holden, Daniel and Saito, Jun and Komura, Taku},
  journal={ACM Transactions on Graphics (TOG)},
  volume={35},
  number={4},
  pages={1--11},
  year={2016},
  publisher={ACM New York, NY, USA}
}

% Simulator 
@article{raisim,
  title={Per-contact iteration method for solving contact dynamics},
  author={Hwangbo, Jemin and Lee, Joonho and Hutter, Marco},
  journal={IEEE Robotics and Automation Letters},
  url="www.raisim.com",
  volume={3},
  number={2},
  pages={895--902},
  year={2018},
  publisher={IEEE}
}

% Navigation Simulators
@inproceedings{szot2021habitat,
  title     =     {Habitat 2.0: Training Home Assistants to Rearrange their Habitat},
  author    =     {Andrew Szot and Alex Clegg and Eric Undersander and Erik Wijmans and Yili Zhao and John Turner and Noah Maestre and Mustafa Mukadam and Devendra Chaplot and Oleksandr Maksymets and Aaron Gokaslan and Vladimir Vondrus and Sameer Dharur and Franziska Meier and Wojciech Galuba and Angel Chang and Zsolt Kira and Vladlen Koltun and Jitendra Malik and Manolis Savva and Dhruv Batra},
  booktitle =     {Advances in Neural Information Processing Systems (NeurIPS)},
  year      =     {2021}
}

@inproceedings{habitat19iccv,
  title     =     {Habitat: {A} {P}latform for {E}mbodied {AI} {R}esearch},
  author    =     {Manolis Savva and Abhishek Kadian and Oleksandr Maksymets and Yili Zhao and Erik Wijmans and Bhavana Jain and Julian Straub and Jia Liu and Vladlen Koltun and Jitendra Malik and Devi Parikh and Dhruv Batra},
  booktitle =     {Proceedings of the IEEE/CVF International Conference on Computer Vision (ICCV)},
  year      =     {2019}
}

@inproceedings{xia2018gibson,
  title={Gibson env: Real-world perception for embodied agents},
  author={Xia, Fei and Zamir, Amir R and He, Zhiyang and Sax, Alexander and Malik, Jitendra and Savarese, Silvio},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={9068--9079},
  year={2018}
}

@article{jain2020pixels,
  title={From pixels to legs: Hierarchical learning of quadruped locomotion},
  author={Jain, Deepali and Iscen, Atil and Caluwaerts, Ken},
  journal={arXiv preprint arXiv:2011.11722},
  year={2020}
}

@inproceedings{fu2022coupling,
  title={Coupling vision and proprioception for navigation of legged robots},
  author={Fu, Zipeng and Kumar, Ashish and Agarwal, Ananye and Qi, Haozhi and Malik, Jitendra and Pathak, Deepak},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={17273--17283},
  year={2022}
}

@article{sorokin2022learning,
  title={Learning to navigate sidewalks in outdoor environments},
  author={Sorokin, Maks and Tan, Jie and Liu, C Karen and Ha, Sehoon},
  journal={IEEE Robotics and Automation Letters},
  volume={7},
  number={2},
  pages={3906--3913},
  year={2022},
  publisher={IEEE}
}



@inproceedings{yokoyama2021success,
  title={Success weighted by completion time: A dynamics-aware evaluation criteria for embodied navigation},
  author={Yokoyama, Naoki and Ha, Sehoon and Batra, Dhruv},
  booktitle={2021 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
  pages={1562--1569},
  year={2021},
  organization={IEEE}
}
@article{kadian2020sim2real,
  title={Sim2real predictivity: Does evaluation in simulation predict real-world performance?},
  author={Kadian, Abhishek and Truong, Joanne and Gokaslan, Aaron and Clegg, Alexander and Wijmans, Erik and Lee, Stefan and Savva, Manolis and Chernova, Sonia and Batra, Dhruv},
  journal={IEEE Robotics and Automation Letters},
  volume={5},
  number={4},
  pages={6670--6677},
  year={2020},
  publisher={IEEE}
}

@article{chaplot2020learning,
  title={Learning to explore using active neural slam},
  author={Chaplot, Devendra Singh and Gandhi, Dhiraj and Gupta, Saurabh and Gupta, Abhinav and Salakhutdinov, Ruslan},
  journal={arXiv preprint arXiv:2004.05155},
  year={2020}
}

@article{hirose2022exaug,
  title={ExAug: Robot-Conditioned Navigation Policies via Geometric Experience Augmentation},
  author={Hirose, Noriaki and Shah, Dhruv and Sridhar, Ajay and Levine, Sergey},
  journal={arXiv preprint arXiv:2210.07450},
  year={2022}
}

@article{carius2019trajectory,
  title={Trajectory optimization for legged robots with slipping motions},
  author={Carius, Jan and Ranftl, Ren{\'e} and Koltun, Vladlen and Hutter, Marco},
  journal={IEEE Robotics and Automation Letters},
  volume={4},
  number={3},
  pages={3013--3020},
  year={2019},
  publisher={IEEE}
}

@inproceedings{cebe2021online,
  title={Online dynamic trajectory optimization and control for a quadruped robot},
  author={Cebe, Oguzhan and Tiseo, Carlo and Xin, Guiyang and Lin, Hsiu-chin and Smith, Joshua and Mistry, Michael},
  booktitle={2021 IEEE International Conference on Robotics and Automation (ICRA)},
  pages={12773--12779},
  year={2021},
  organization={IEEE}
}

@article{li2022ganimator,
  title={GANimator: Neural Motion Synthesis from a Single Sequence},
  author={Li, Peizhuo and Aberman, Kfir and Zhang, Zihan and Hanocka, Rana and Sorkine-Hornung, Olga},
  journal={arXiv preprint arXiv:2205.02625},
  year={2022}
}



@article{howe1999bayesian,
  title={Bayesian reconstruction of 3d human motion from single-camera video},
  author={Howe, Nicholas and Leventon, Michael and Freeman, William},
  journal={Advances in neural information processing systems},
  volume={12},
  year={1999}
}

@article{safonova2004synthesizing,
  title={Synthesizing physically realistic human motion in low-dimensional, behavior-specific spaces},
  author={Safonova, Alla and Hodgins, Jessica K and Pollard, Nancy S},
  journal={ACM Transactions on Graphics (ToG)},
  volume={23},
  number={3},
  pages={514--521},
  year={2004},
  publisher={ACM New York, NY, USA}
}

@incollection{kovar2008motion,
  title={Motion graphs},
  author={Kovar, Lucas and Gleicher, Michael and Pighin, Fr{\'e}d{\'e}ric},
  booktitle={ACM SIGGRAPH 2008 classes},
  pages={1--10},
  year={2008}
}

@inproceedings{mizuguchi2001data,
  title={Data driven motion transitions for interactive games.},
  author={Mizuguchi, Mark and Buchanan, John and Calvert, Tom},
  booktitle={Eurographics (Short Presentations)},
  year={2001}
}

@article{rose1998verbs,
  title={Verbs and adverbs: Multidimensional motion interpolation},
  author={Rose, Charles and Cohen, Michael F and Bodenheimer, Bobby},
  journal={IEEE Computer Graphics and Applications},
  volume={18},
  number={5},
  pages={32--40},
  year={1998},
  publisher={IEEE}
}

%% Robots
@misc{unitree,
title={Unitree robotics},
note={http://www.unitree.cc/}
}

%% Optimizers
% IFOPT in TOWR
@misc{ifopt,
  author       = {Alexander W Winkler},
  title        = {{Ifopt - A modern, light-weight, Eigen-based C++ interface to 
                   Nonlinear Programming solvers Ipopt and Snopt.}},
  year         = 2018,
  doi          = {10.5281/zenodo.1135046},
  url          = {https://doi.org/10.5281/zenodo.1135046}
}
% IPOPT in TOWR
@article{wachter2006implementation,
  title={On the implementation of an interior-point filter line-search algorithm for large-scale nonlinear programming},
  author={W{\"a}chter, Andreas and Biegler, Lorenz T},
  journal={Mathematical programming},
  volume={106},
  pages={25--57},
  year={2006},
  publisher={Springer}
}



%%%%%% Visual Locomotion Citation %%%%%%%%%%%
@article{kumar2021rma,
  title={Rma: Rapid motor adaptation for legged robots},
  author={Kumar, Ashish and Fu, Zipeng and Pathak, Deepak and Malik, Jitendra},
  journal={arXiv preprint arXiv:2107.04034},
  year={2021}
}
@inproceedings{yu2021visual,
  title={Visual-locomotion: Learning to walk on complex terrains with vision},
  author={Yu, Wenhao and Jain, Deepali and Escontrela, Alejandro and Iscen, Atil and Xu, Peng and Coumans, Erwin and Ha, Sehoon and Tan, Jie and Zhang, Tingnan},
  booktitle={5th Annual Conference on Robot Learning},
  year={2021}
}
@article{jenelten2020perceptive,
  title={Perceptive locomotion in rough terrain--online foothold optimization},
  author={Jenelten, Fabian and Miki, Takahiro and Vijayan, Aravind E and Bjelonic, Marko and Hutter, Marco},
  journal={IEEE Robotics and Automation Letters},
  volume={5},
  number={4},
  year={2020},
  publisher={IEEE}
}
@article{grandia2022perceptive,
  title={Perceptive locomotion through nonlinear model predictive control},
  author={Grandia, Ruben and Jenelten, Fabian and Yang, Shaohui and Farshidian, Farbod and Hutter, Marco},
  journal={arXiv preprint arXiv:2208.08373},
  year={2022}
}

%%% Experiment Settings %%%
@article{paszke2019pytorch,
  title={Pytorch: An imperative style, high-performance deep learning library},
  author={Paszke, Adam and Gross, Sam and Massa, Francisco and Lerer, Adam and Bradbury, James and Chanan, Gregory and Killeen, Trevor and Lin, Zeming and Gimelshein, Natalia and Antiga, Luca and others},
  journal={Advances in neural information processing systems},
  volume={32},
  year={2019}
}

@article{coumans2016pybullet,
  title={Pybullet, a python module for physics simulation for games, robotics and machine learning},
  author={Coumans, Erwin and Bai, Yunfei},
  year={2016}
}
@article{schulman2017proximal,
  title={Proximal policy optimization algorithms},
  author={Schulman, John and Wolski, Filip and Dhariwal, Prafulla and Radford, Alec and Klimov, Oleg},
  journal={arXiv preprint arXiv:1707.06347},
  year={2017}
}

%%% RRT* %%%
@article{karaman2011sampling,
  title={Sampling-based algorithms for optimal motion planning},
  author={Karaman, Sertac and Frazzoli, Emilio},
  journal={The international journal of robotics research},
  volume={30},
  number={7},
  pages={846--894},
  year={2011},
  publisher={Sage Publications Sage UK: London, England}
}

%% NavMesh
@inproceedings{van2016comparative,
  title={A comparative study of navigation meshes},
  author={Van Toll, Wouter and Triesscheijn, Roy and Kallmann, Marcelo and Oliva, Ramon and Pelechano, Nuria and Pettr{\'e}, Julien and Geraerts, Roland},
  booktitle={Proceedings of the 9th International Conference on Motion in Games},
  pages={91--100},
  year={2016}
}

%% Training Details
% ELU
@article{clevert2015fast,
  title={Fast and accurate deep network learning by exponential linear units (elus)},
  author={Clevert, Djork-Arn{\'e} and Unterthiner, Thomas and Hochreiter, Sepp},
  journal={arXiv preprint arXiv:1511.07289},
  year={2015}
}

@article{bisong2019google,
  title={Google colaboratory},
  author={Bisong, Ekaba and Bisong, Ekaba},
  journal={Building machine learning and deep learning models on google cloud platform: a comprehensive guide for beginners},
  pages={59--64},
  year={2019},
  publisher={Springer}
}
% \bibitem{c3} H. Poor, An Introduction to Signal Detection and Estimation.   New York: Springer-Verlag, 1985, ch. 4.
% \bibitem{c4} B. Smith, ÒAn approach to graphs of linear forms (Unpublished work style),Ó unpublished.
% \bibitem{c5} E. H. Miller, ÒA note on reflector arrays (Periodical styleÑAccepted for publication),Ó IEEE Trans. Antennas Propagat., to be publised.
% \bibitem{c6} J. Wang, ÒFundamentals of erbium-doped fiber amplifiers arrays (Periodical styleÑSubmitted for publication),Ó IEEE J. Quantum Electron., submitted for publication.
% \bibitem{c7} C. J. Kaufman, Rocky Mountain Research Lab., Boulder, CO, private communication, May 1995.
% \bibitem{c17} J. G. Kreifeldt, ÒAn analysis of surface-detected EMG as an amplitude-modulated noise,Ó presented at the 1989 Int. Conf. Medicine and Biological Engineering, Chicago, IL.
% \bibitem{c18} J. Williams, ÒNarrow-band analyzer (Thesis or Dissertation style),Ó Ph.D. dissertation, Dept. Elect. Eng., Harvard Univ., Cambridge, MA, 1993. 
% \bibitem{c19} N. Kawasaki, ÒParametric study of thermal and chemical nonequilibrium nozzle flow,Ó M.S. thesis, Dept. Electron. Eng., Osaka Univ., Osaka, Japan, 1993.
% \bibitem{c20} J. P. Wilkinson, ÒNonlinear resonant circuit devices (Patent style),Ó U.S. Patent 3 624 12, July 16, 1990. 






\end{thebibliography}

